Planning and Perception for Unmanned Aerial Vehicles in Object and Environmental Monitoring

Unmanned Aerial Vehicles (UAVs) equipped with high-resolution sensors enable extensive data collection from previously inaccessible areas at a remarkable spatio-temporal scale, promising to revolutionize fields such as precision agriculture and infrastructure inspection. To fully exploit their potential, developing autonomy algorithms for planning and perception is crucial. This dissertation focuses on developing planning and perception algorithms tailored to UAVs used in monitoring applications. In the first part, we address object monitoring and its associated planning challenges. Object monitoring involves continuous observation, tracking, and analysis of specific objects. We tackle the problem of visual reconstruction where the goal is to maximize visual coverage of an object in an unknown environment efficiently. Leveraging shape prediction deep learning models, we optimize planning for quick information gathering. Extending this to multi-UAV systems, we create efficient paths around objects based on reconstructed 3D models, crucial for close-up inspections aimed at detecting changes. Next, we explore inspection scenarios where an object has changed or no prior information is available, focusing on infrastructure inspection. We validate our planning algorithms through real-world experiments and high-fidelity simulations, integrating defect detection seamlessly into the process. In the second part, we shift focus to monitoring entire environments, distinct from object-specific monitoring. Here, the goal is to maximize coverage to understand spatio-temporal changes. We investigate slow-changing environments like vegetative growth estimation and fast-changing environments such as wildfire management. For wildfires, we employ informative path planning to validate and localize fires early, utilizing LSTM networks for enhanced early detection.

==> Abbreviations-supertabular.tex <==
%List of Abbreviations


\renewcommand{\baselinestretch}{1}
\small\normalsize
\hbox{\ }

\vspace{.5in}

\begin{center}
\large{List of Abbreviations}
\end{center} 

\vspace{3pt}

\begin{supertabular}{ll}
Add later & if needed \\
%$\alpha$ & alpha \\
%$\beta$  & beta \\
&  \\ 
%IREAP & Institute for Research in Electronics and Applied Physics \\
%NSA & National Security Agency
\end{supertabular}


==> Abbreviations.tex <==
%List of Abbreviations

\renewcommand{\baselinestretch}{1}
\small\normalsize
\hbox{\ }

\vspace{.5in}


\begin{center}
\large{List of Abbreviations}
\end{center} 

\vspace{3pt}

\begin{tabular}{ll}
$\alpha$ & alpha \\
$\beta$  & beta \\
&  \\ 
IREAP & Institute for Research in Electronics and Applied Physics \\
NSA & National Security Agency
\end{tabular}


==> Bibliography.tex <==
\begin{thebibliography}{99}
\setlength{\parskip}{1em}

\bibitem{Agrawal1} G.P. Agrawal, {\em Nonlinear Fiber Optics} (Academic
Press, San Diego, CA, 2001), Chap. 1.
\bibitem{Bloembergen} N. Bloembergen, {\em Nonlinear Optics} (Benjamin,
Reading, MA, 1977).
\bibitem{Shen} Y.R. Shen, {\em Principles of Nonlinear Optics} (Wiley, New
York, 1984).
\bibitem{Butcher} P.N. Butcher and D.N. Cotter, {\em The Elements of
Nonlinear Optics} (Cambridge University Press, Cambridge, UK, 1990).
\bibitem{Boyd} R.W. Boyd, {\em Nonlinear Optics} (Academic Press, San Diego,
CA, 1992).
\bibitem{Newell} A.C. Newell and J.V. Moloney {\em Nonlinear Optics (Advanced Topics in the Interdisciplinary Mathematical Sciences)} (Westview Press, Boulder, CO, April 1992). 
\bibitem{Marcuse} D. Marcuse,{\em Light Transmission Optics} (Van Nostrand
Reinhold, New York, 1982), Chaps. 8 and 12.
\bibitem{Agrawal2} G.P. Agrawal, {\em Nonlinear Fiber Optics} (Academic
Press, San Diego, CA, 2001), Chap. 2.
\bibitem{Diament} P. Diament, {\em Wave Transmission and Fiber Optics}
(Macmillan, New York, 1990).
\bibitem{Zakharov} V.E. Zakharov and A.Shabat, Sov. Phys. JETP 
\textbf{34}, 62 (1972)
\bibitem{Hardin} R.H. Hardin and F.D. Tappert, SIAM
Rev. Chronicle \textbf{15}, 423 (1973).
\bibitem{Fisher} R.A.Fisher and
W.K. Bischel, Appl. Phys. Lett. \textbf{23}, 661 (1973); J. Appl. Phys
\textbf{46}, 4921 (1975).
\bibitem{Cooley} J.W. Cooley and J.W. Tukey,
Math. Comput. \textbf{19}, 297 (1965).
\bibitem{Trebino} R. Trebino, D.J. Kane, "Using phase retrieval to measure
the intensity and phase of ultrashort pulses: frequency resolved optical gating," J. Opt. Soc. Am. B \textbf{10}, 1101 (1993). 
\bibitem{Kanejqe} D.J. Kane, R. Trebino, "Characterization of Arbitrary Femtosecond Pulses Using Frequency-Resolved Optical Gating," IEEE J. Quant. Elect. \textbf{29}, 571 (1993). 
\bibitem{Kaneoptlett} D.J. Kane, R. Trebino, "Single-shot measurement of the intensity and phase of an arbitrary ultrashort pulse  by using frequency-resolved optical gating," Opt. Lett. \textbf{10}, 1101 (1993).
\bibitem{OShealett}P. O'Shea, M. Kimmel, X. Gu, R. Trebino, "Highly simplified device for ultrashort-pulse measurement," Opt. Lett. \textbf{26}, 932 (2001).
\bibitem{Agrawal3} G.P. Agrawal, {\em Nonlinear Fiber Optics} (Academic
Press, San Diego, CA, 2001), Chap. 3.
\bibitem{Agrawal4} G.P. Agrawal, {\em Nonlinear Fiber Optics} (Academic
Press, San Diego, CA, 2001), Chap. 4.
\bibitem{Agrawal10} G.P. Agrawal, {\em Nonlinear Fiber Optics} (Academic
Press, San Diego, CA, 2001), Chap. 10.
\bibitem{Agrawal7} G.P. Agrawal, {\em Nonlinear Fiber Optics} (Academic
Press, San Diego, CA, 2001), Chap. 7.
\bibitem{Agrawal6} G.P. Agrawal, {\em Nonlinear Fiber Optics} (Academic
Press, San Diego, CA, 2001), Chap. 6.
\bibitem{Stolen} R.H. Stolen, E.P. Ippen, and A.R. Tynes,
Appl. Phys. Lett. \textbf{20}, 62 (1972). 
\bibitem{Ippen} E.P. Ippen and R.H. Stolen, Appl. Phys. Lett. \textbf{21}, 
539 (1972). 
\bibitem{Smith} R.G. Smith, Appl. Opt. \textbf{11}, 2489 (1972).
\bibitem{Agrawal9} G.P. Agrawal, {\em Nonlinear Fiber Optics} (Academic
Press, San Diego, CA, 2001), Chap. 9.
\bibitem{Agrawal8} G.P. Agrawal, {\em Nonlinear Fiber Optics} (Academic
Press, San Diego, CA, 2001), Chap. 8.
\bibitem{hart1} D.L. Hart, Arthur F. Judy, Rajarshi Roy and James W. Beletic, Phys. Rev. E \textbf{57}, 4757 (1998); D.L. Hart, Arthur F. Judy, T.A.B. Kennedy, Rajarshi Roy and K. Stoev, Phys. Rev. A \textbf{50}, 1807 (1994).   
\bibitem{ito} K. Ito, {\em Lectures on Stochastic Processes} (Tata Institute of Fundamental Research, Bombay, 1960).
\bibitem{stratanovich} R.L. Stratanovich, {\em Topics in the Theory of Random Noise}, Vols I. and II. (Gordon \& Breach, New York, 1963).
\bibitem{risken} H. Risken, {\em The Fokker-Planck Equation} (Springer-Verlag, Berlin, 1989).
\bibitem{werner2} M.J. Werner and P.D. Drummond, J. Comput. Phys. \textbf{132}, 312 (1997).
\bibitem{drummond1} P.D. Drummond and I.K. Mortimer, J. Comput. Phys. \textbf{93}, 144 (1991).
\bibitem{carter3} S.J. Carter, Phys. Rev. A. \textbf{51}, 3274 (1995).
\bibitem{thompson1} J.R. Thompson and Rajarshi Roy, Phys. Rev. A \textbf{43}, 4987 (1991).
\bibitem{boxmuller} W.H. Press, S.A. Teukolsky, W.T. Vetterling and B.P. Flannery, {\em Numerical Recipes in Fortran: The Art of Scientific Computing} (Cambridge University Press, Cambridge, 1992).
\bibitem{headley} C. Headley, G.P. Agrawal, IEEE J. Quantum Electron. \textbf{QE-31}, 2058 (1995), C. Headley, G.P. Agrawal J. Opt. Soc. Am. B. \textbf{13}, 2170 (1995).
\bibitem{perlmutter1} S.H. Perlmutter, M.D. Levenson, R.M. Shelby and
M.B. Weisman, Phys. Rev. Lett. \textbf{61} 1388, 1988.
\bibitem{abdullaev} F. Kh. Abdullaev, J.H. Hensen, S. Bischoff and M.P. Sorensen, J. Opt. Soc. Am. B. \textbf{15}, 2424 (1998); F. Kh. Abdullaev, J.G. Caputo, and Nikos Flytzanis, Phys. Rev E. \textbf{50}, 1552 (1994).
\bibitem{glenn} William H. Glenn, IEEE J. Quantum Electron. \textbf{QE-25}, 1218 (1989).
\bibitem{Trebinobook} R. Trebino. {\em Frequency-Resolved Optical Gating: The Measurement of Ultrashort Laser Pulses} (Kluwer Academic 2002).
\bibitem{Agrawal} G.P. Agrawal {\em Nonlinear Fiber Optics} (Academic,
San Diego, 2001).
\bibitem{Dudley} J.M. Dudley, X. Gu, L. Xu, M. Kimmel, E. Zeek, P. O'Shea, R. Trebino, S. Coen, R.S. Windeler, "Cross-correlation frequency resolved optical gating analysis of broadband continuum generation in photonic crystal fiber: simulations and experiments," Opt. Express \textbf{10}, 1215 (2002).
\bibitem{Liu1} Q.D. Liu, J.T. Chen, Q.Z. Wang, P.P. Ho, and R.R. Alfano, "Single pulse degenerate-cross-phase modulation in a single-mode optical fiber," Opt. Lett. \textbf{20}, 542 (1995).
\bibitem{Sylvestre} T. Sylvestre, H. Maillotte, E. Lantz, and D. Gindre "Combined spectral effects of pulse walk-off and degenerate cross-phase modulation in birefringent fibers", Journal of Nonlinear Optical Physics and Materials 6, 313-320 (1997).
\bibitem{Liu2} Q.D. Liu, L. Shi, P.P. Ho, R.R. Alfano, R.J. Essiambre, and G.P. Agrawal, "Degenerate cross-phase modulation of femtosecond laser pulses in a birefringent single-mode fiber," IEEE Photon. Tech. Lett. \textbf{9}, 1107 (1997). 
\bibitem{Omenetto1} F.G. Omenetto, B.P. Luce, D. Yarotski and A.J. Taylor, "Observation of chirped soliton dynamics at l= 1.55 mm in a single-mode optical fiber with frequency-resolved optical gating," Opt. Lett. \textbf{24}, 1392 (1999).
% 1.55 micron regime - check for more recent papers by Omenetto use both web-sci and inspec
\bibitem{Omenetto2} F.G. Omenetto, Y. Chung, D. Yarotski, T. Shaefer, I. Gabitov and A.J. Taylor, "Phase analysis of nonlinear femtosecond pulse propagation and self-frequency shift in optical fibers," Opt. Commun. \textbf{208}, 191 (2002). 
\bibitem{Omenetto3} F.G. Omenetto, J.W. Nicholson, B.P. Luce, D. Yarotski, A.J. Taylor, "Shaping, propagation and characterization of ultrafast pulses in optical fibers," Appl. Phys. B \textbf{70}[Suppl.], S143 (2000).
\bibitem{Nishizawa1} N. Nishizawa and T. Goto, "Experimental analysis of ultrashort pulse propagation in optical fibers around zero-dispersion region using cross-correlation frequency resolved optical gating," Opt. Express \textbf{8}, 328 (2001).
\bibitem{Nishizawa2} N. Nishizawa and T. Goto, "Trapped pulse generation by femtosecond soliton pulse in birefringent optical fibers," Opt. Express \textbf{10}, 256 (2002).
\bibitem{Nishizawa3} N. Nishizawa and T. Goto, "Characteristics of pulse trapping by use of ultrashort soliton pulses in optical fibers across the zero-dispersion wavelength," Opt. Express \textbf{10}, 1151 (2002).
\bibitem{Nishizawa4} N. Nishizawa and T. Goto, "Ultrafast all optical switching by use of pulse trapping across zero-dispersion wavelength," Opt. Express \textbf{11}, 359 (2003).
% All of Nishizawa and Goto papers are related to 1.3 micron experiments and simulations.
\bibitem{Ogawa}, K. Ogawa, M.D. Pelusi, "Characterization of ultrashort optical pulses in a dispersion-managed fiber link using two-photon absorption frequency-resolved optical gating," Opt. Commun. \textbf{198}, 83-87 (2001).
\bibitem{Altes} R.A. Altes, "Detection, estimation, and classification
with spectrograms," J. Acoust. Soc. Am. \textbf{67}(4), 1232 (1980).
\bibitem{Christian} A. Christian Silva, "GRENOUILLE - Practical Issues," unpublished.
\bibitem{Mejia} J. Garduno-Mejia, A.H. Greenaway, and D.T. Reid, "Designer
femtosecond pulses using adaptive optics," Opt. Express \textbf{11}
2030 (2003).
\bibitem{OSheaexpress1} P. O'Shea, M. Kimmel, X. Gu, R. Trebino, "Increased-bandwidth in ultrashort-pulse measurement using an angle-dithered nonlinear-optical crystal," Opt. Express \textbf{7}, 342 (2000).
\bibitem{OSheaexpress2} P. O'Shea, M. Kimmel, R. Trebino, "Increased phase-matching bandwidth in simple ultrashort-laser-pulse measurements," J. Opt. B \textbf{4}, 44 (2002).
\bibitem{Akturk} S. Akturk, M. Kimmel, P. O'Shea, R. Trebino, "Measuring pulse-front tilt in ultrashort pulses using GRENOUILLE", Opt. Express \textbf{11}, 491 (2003).
\bibitem{Blow} K. J. Blow, D. Wood, "Theoretical Description of Transient Stimulated Raman Scattering in Optical Fibers," IEEE J. Quant. Elect. \textbf{25}, 2665 (1989).
\bibitem{Stolen2} R.H. Stolen, J.P. Gordon, W.J. Tomlinson,
J. Opt. Soc. Am. B \textbf{6}, 1159 (1989).
\bibitem{Mamyshev} P.V. Mamyshev and S.V. Chernikov, Sov. Lightwave
Commun. \textbf{2}, 97 (1992).
\bibitem{Headleythesis} C. Headley III, \em{Ultrafast Stimulated Raman
Scattering in Optical Fibers}, Ph.D. Thesis, University of Rochester,
NY (1995).
\end{thebibliography}


==> Foreword.tex <==
%Foreword

\renewcommand{\baselinestretch}{2}
\small\normalsize
\hbox{\ }
 
\vspace{.5in}

\begin{center}
\large{Foreword} 
\end{center} 

If needed.


==> Preface.tex <==
%Preface
\pagestyle{plain}\pagenumbering{roman} \setcounter{page}{2}
\renewcommand{\baselinestretch}{2}
\small\normalsize
\hbox{\ }

\vspace{.5in}

\begin{center}
\large{Preface}
\end{center}


If needed.

